A theory on power in networks

The eigenvector centrality equation $\lambda x = A \, x$ is a successful compromise between simplicity and expressivity. It claims that central actors are those connected with central others. For at least 70 years, this equation has been explored in disparate contexts, including econometrics, sociometry, bibliometrics, Web information retrieval, and network science. We propose an equally elegant counterpart: the power equation $x = A x^{\div}$, where $x^{\div}$ is the vector whose entries are the reciprocal of those of $x$. It asserts that power is in the hands of those connected with powerless others. It is meaningful, for instance, in bargaining situations, where it is advantageous to be connected to those who have few options. We tell the parallel, mostly unexplored story of this intriguing equation.

==> experiments.tex <==
\section{Experiments} \label{experiments}

In this section we experiment with power on real social networks. We concocted the following assessments:

\begin{itemize}

\item \emph{Efficiency}. We measure how fast is to compute power, both in the original and perturbed versions, using the computation of centrality as a benchmark.

\item \emph{Quality}. We verify how much perturbed power differs from the original one.

\item \emph{Novelty}. We investigate the correlation of power with other centrality and power measures.
\end{itemize}

In the above illustrated experiments we used the following social networks: \emph{Dolphin}: a social network among dolphins \cite{LN04}; \emph{Madrid}: the Madrid train bombing terrorist network \cite{H06}; \emph{Jazz}: a social network of Jazz musicians \cite{GD03}; \emph{Karate}: a network of friendships between members of a karate club \cite{Z77}; \emph{Collaboration}: a collaboration network of scholars in the field of network science \cite{NG04}; \emph{Karenina}: a co-appearance network of characters in the novel Anna Karenina by Lev Tolstoj \cite{K93}.
It is worth pointing out that the designed experiments are not influenced by the size of the network.


\subsection{Efficiency}

In this assessment, we measure the complexity of computation of power. We use both Sinkhorn-Knopp method (SK for short) and Newton method\footnote{For this method we used the code provided in \cite{KR13}.} (NM for short). We consider the computation on the original matrix as well as on the perturbed ones. We use as a benchmark the complexity of the computation of centrality using the power method (PM for short). The complexity is expressed as the number of  matrix-vector product operations. If a matrix is sparse (this is the case for all tested networks), such operation has linear complexity in the number of nodes of the graph.
%In all methods we use a precision of $10^{-6}$.


The main empirical findings are summarized in the following (see Table \ref{statistics} and Figures \ref{exp1-diagonal}, \ref{exp1-full} and \ref{exp1-diagonalNewton}):

\begin{enumerate}
\item  SK on the original matrix is significantly slower than PM;

\item as predicted by theory, the speed of the SK method is associated with the magnitude of the second largest eigenvalue of the bistochastic matrix: the closer the eigenvalue to $1$, the higher the complexity of the SK method;

\item diagonal perturbation does not significantly change the speed of SK. Moreover, an increase in the damping parameter has a non-monotonic effect on the speed of SK: the complexity may increase, decrease, or stay stable, depending on the structure of the graph matrix;

\item on the other hand, full perturbation does significantly increase the speed of SK so that the complexity of SK with full perturbation and that of PM are comparable. Furthermore, an increase in the damping parameter has a monotonic effect on the speed of SK: the larger the damping parameter, the faster the method;

\item NM on the original matrix is much faster than SK; its complexity is comparable to that of fully perturbed SK and PM;


\item NM with diagonal perturbation is even faster than NM and an increase in the damping parameter in the diagonal perturbation has a monotonic effect on the speed of NM: the larger the damping parameter, the faster the method.

\end{enumerate}








\subsection{Quality}

This assessment investigates the quality of perturbed power (power computed on a perturbed adjacency matrix). We measure quality as Pearson correlation between original and perturbed power solutions. The closer the correlation to 1, the closer the perturbed solution to the original one, hence the higher the quality of the perturbed solution.

The outcomes of this experiment are summarized in the following, see  Figure \ref{exp2-compare}:

\begin{enumerate}
\item as soon as the damping parameter is small, both diagonal and full perturbations do not significantly change the original power;

\item power with diagonal perturbation is closer to original power than power with full perturbation;

\item the larger the damping parameter, the lower the quality of solutions for both perturbations.
\end{enumerate}






\subsection{Novelty}

In this assessment we explore the overlapping of power with both centrality and degree. In particular, we use \textit{partial correlation} to evaluate the actual association among power and centrality, excluding the inherent effect that degree has on both measures. Moreover, we compare power with Bonacich power (Bonacich index with negative $\beta$).

The main empirical outcomes are summarized in the following, see Tables \ref{exp3.correlation} and \ref{exp3.ranking} and Figure \ref{exp3-Bonacich}:

\begin{enumerate}
\item both power and centrality are positively correlated with degree;
\item power is, however, negatively correlated with centrality when the effect of degree is excluded;
\item power is positively correlated with Bonacich power and the correlations increases as the parameter $\beta$ declines below $0$. The association is higher when the adjacency matrix is perturbed.
\end{enumerate}





\begin{comment}

\subsection{Sum-up}

We bumped into the well-known trade-off between efficiency and effectiveness. On one side of the spectrum, the most effective solution is power computed on the original network, without introducing any artificial perturbation of the network topology. However, such a solution is either diverging (when the graph is not regularizable) or its computation is slow. On the other side of the spectrum, the most efficient solution is power computed on a heavily perturbed matrix. However, such a matrix is far from the original topology of the network, hence the resulting power is not telling the truth. We suggest a balanced compromise between these two extremes: full perturbation with a small damping parameter.

Diagonal perturbation is a less invasive disturbance of the network with respect to full perturbation, since it modifies less elements. In particular diagonal perturbation changes only elements on the diagonal of the matrix, increasing in this way the self-confidence of each actor of the system and leaving unchanged the strength of the relation between any two actors. Unfortunately, we experienced that diagonal perturbation does not speed up in a significative way the computation of power using the Sinkhorn-Knopp method. This might be not the case with Newton method, however. Recall that the first iteration of Newton method for the computation of power corresponds to Bonacich power (Bonacich index with negative $\beta$). Figure \ref{exp3-Bonacich} suggests that Newton method converges in less outer iterations (hence faster) on perturbed matrices, independently on the type of perturbation (diagonal or full). Hence, diagonally perturbed power might represent an effective as well as efficient solution as soon as Newton method in employed for the computation.

Finally, power is not centrality: there are significant divergences among the two measures. As soon as the effect of degree is ruled out, power is negatively associated with centrality. On the other hand, power is positively correlated with both degree centrality and Bonacich power. This is not very surprising, since degree centrality and Bonacich power are the outcomes of the first iteration of, respectively, the Sinkhorn-Knopp method and the Newton method for the computation of power. In this view, power can be regarded as a more accurate measure than its first-iteration approximations.

\end{comment}

